Proton and Neutron Irradiation Tests of Readout Electronics of the ATLAS Hadronic Endcap Calorimeter

The readout electronics of the ATLAS Hadronic Endcap Calorimeter will have to withstand the about ten times larger radiation environment of the future high-luminosity LHC (HL-LHC) compared to their design values. The GaAs ASIC which comprises the heart of the readout electronics has been exposed to neutron and proton radiation with fluences up to ten times the total expected fluences for ten years of running of the HL-LHC. Neutron tests were performed at the NPI in Rez, Czech Republic, where a 36 MeV proton beam is directed on a thick heavy water target to produce neutrons. The proton irradiation was done with 200 MeV protons at the PROSCAN area of the Proton Irradiation Facility at the PSI in Villigen, Switzerland. In-situ measurements of S-parameters in both tests allow the evaluation of frequency dependent performance parameters - like gain and input impedance - as a function of the fluence. The linearity of the ASIC response has been measured directly in the neutron tests with a triangular input pulse of varying amplitude. The performance measurements and expected performance degradations under HL-LHC conditions are presented.

==> PaxHeaders.30351/ieee2012proc.tex <==
30 mtime=1353075308.114396921
30 atime=1353075316.182359987
30 ctime=1353075308.114396921

